How I failed machine learning in medical imaging -- shortcomings and recommendations

Medical imaging is an important research field with many opportunities for improving patients' health. However, there are a number of challenges that are slowing down the progress of the field as a whole, such optimizing for publication. In this paper we reviewed several problems related to choosing datasets, methods, evaluation metrics, and publication strategies. With a review of literature and our own analysis, we show that at every step, potential biases can creep in. On a positive note, we also see that initiatives to counteract these problems are already being started. Finally we provide a broad range of recommendations on how to further these address problems in the future. For reproducibility, data and code for our analyses are available on \url{https://github.com/GaelVaroquaux/ml_med_imaging_failures}

==> cover.tex <==
I think one thing might be is that we read wider and incorporate findings from areas related to ML (and not just the main AI in medicine venues for example)
5:36 PM
Yes, and we give technical explainations and solutions. We need however to be careful with this line, as it may play against us to publish in a medical journal

https://www.nature.com/npjdigitalmed/about/editors

recent editorial!!

\gv{Positioning of the paper (to keep in mind in the framing, title, and letter to the editor): methodological shortcomings, as opposed to domain
ones, for instance not inserting the AI in the right slot in the clinical
process. We need to frame properly our paper here to position ourselves
with other papers, and to leverage properly our expertise}


%---------DONE
% Fix Excel figure to Python - VC - DONE
% Draft section on evaluation error - VC - DONE
% Check author guidelines Natural Digital Medicine - VC - DONE 

% https://www.nature.com/documents/npj-submission-guide.pdf 
% https://www.nature.com/documents/npj-gta.pdf


% Author order - DONE (GV, VC)
% Check if arXiV papers have recent published versions - Done

%---------TODO


% Post on arXiV for Veronika's grant - VC



% Ask Sylvia Villeneuve to read  - GV
% Ask a colleague to read  - VC
% Open access fee
% Review consistency of terminology used

% Choose "content type" (Article/perspective) https://www.nature.com/npjdigitalmed/about/content-types/

% Write cover letter

% Check word counts etc (abstract 150, main text 5K for articles, 10 figures/tables, 70 references)

% Avoid 'Introduction' as a heading

% For all statistics (including error bars), provide the EXACT n values used to calculate the statistics 

% Data availability statement (before References)
% 


% Reviewers - GV 
% - L Oakden-Rayner
% - Zach Lipton
% - HughHarvey https://twitter.com/DrHughHarvey
% - Marzyeh Ghassemi
% - Andrew Beam https://www.hsph.harvard.edu/andrew-beam/
% - Brett Beaulieu-Jones
% - Nikola Stikov https://scholar.google.ca/citations?user=02a5TU8AAAAJ&hl=en

